A Feasibility-Seeking Approach to Two-stage Robust Optimization in Kidney Exchange

Kidney paired donation programs (KPDPs) match patients with willing but incompatible donors to compatible donors with an assurance that when they donate, their intended recipient receives a kidney in return from a different donor. A patient and donor join a KPDP as a pair, represented as a vertex in a compatibility graph, where arcs represent compatible kidneys flowing from a donor in one pair to a patient in another. A challenge faced in real-world KPDPs is the possibility of a planned match being cancelled, e.g., due to late detection of organ incompatibility or patient-donor dropout. We therefore develop a two-stage robust optimization approach to the kidney exchange problem wherein (1) the first stage determines a kidney matching solution according to the original compatibility graph, and then (2) the second stage repairs the solution after observing transplant cancellations. In addition to considering homogeneous failure, we present the first approach that considers non-homogeneous failure between vertices and arcs. To this end, we develop solution algorithms with a feasibility-seeking master problem and evaluate two types of recourse policies. Our framework outperforms the state-of-the-art kidney exchange algorithm under homogeneous failure on publicly available instances. Moreover, we provide insights on the scalability of our solution algorithms under non-homogeneous failure for two recourse policies and analyze their impact on highly-sensitized patients, patients for whom few kidney donors are available and whose associated exchanges tend to fail at a higher rate than non-sensitized patients.

==> 8_PaperOutline.tex <==
\section{Paper outline}

\begin{itemize}
    \item Introduction
    \begin{itemize}
        \item Motivation
        \item Contribution
    \end{itemize}
    \item Problem Description
        \begin{itemize}
        \item Non-homogeneous failure $\rightarrow$ Define uncertainty set
        \item Recourse policies (add examples)
        \item Generic RO model distinguishing the two decision stages
        \item Solving the RO model via delayed-scenario generation, using notation of the two stages (show algorithm as in Carvalho 2021)
    \end{itemize}
    \item First-stage formulation for the full-recourse policy and the new one (same formulation, show slight changes)
        \item Solving second-stage as an interdiction problem
        \begin{itemize}
            \item A Basic Covering Decomposition
            \begin{itemize}
                \item Show Bloom,2021 second-stage reformulation adapted to non-homogeneous uncertainty
                \item Show our new second-stage reformulation
                \item Proof of equivalence between our reformulation and that in Bloom,2021
                \item Basic covering algorithm (show algorithm)
            \end{itemize}
            \item An Enhanced Covering Decomposition
            \begin{itemize}
                \item Lifting covering constraints
                \begin{itemize}
                    \item Show proof
                    \item Show example
                \end{itemize}
                \item Other super-valid inequalities
                (SVIs)--- show proofs, figures and how to compute them for every recourse policy, 
                \begin{itemize}
                    \item Vertex for Vertex
                    \item Vertex for Arc
                    \item Arc for Vertex
                    \item Arc for Arc (tricky to compute, may not include it)
                \end{itemize}
                \item Solving the MP (covering problem) heuristically
                \item Enhanced covering algorithm (SVIs + heuristic)
            \end{itemize}
            %\item Solving MP as MAXSAT problem (\textcolor{blue}{ideally!})
            %\begin{itemize}
            %    \item Show formulation
            %    \item Show SVIs in Conjunctive Normal Form (CNF)
            %\end{itemize}
        \end{itemize}
        \item Solution methodology
            \begin{itemize}
                \item Connect the first and second stage solution methodologies
                \item Show final solution algorithm for each recourse policy?
            \end{itemize}
        \item Computational Experiments
            \begin{itemize}
                \item Methodological comparison
                \begin{itemize}
                    \item Compare Bloom,2021 and our work for the full-recourse policy
                    \item Comparison of the Basic Covering, the Enhanced Covering and the MAXSAT+Enhanced Covering
                    \item For the best version of our algorithm, change the cycle/chain/graph size and compare.  
                \end{itemize}
                \item Solution comparison
                \begin{itemize}
                    \item Recourse policies comparison
                    \item Sensitivity analysis on problem parameters (K,L, vertex and arc budget)
                 \end{itemize}   
            \end{itemize}
\end{itemize}

Singleton donors, which can be classified as \textit{altruistic} donors, \textit{bridge} donors or even \textit{deceased} donors, can also register in a \KPDP. Their goal is to donate one of their two kidneys to a patient in need without expecting a swap in return. After determining compatible exchanges, some patients are selected for transplantation following the \KPDP's prioritization policies. Such compatibilities can be expressed in a directed graph (compatibility graph), where vertices represent either a pair or a singleton donor, and an arc exists between two vertices if the donor from one pair is compatible with the patient in another pair. The direction of the arc indicates the direction of donated organ flow. Such transplants take the form of simple cycles when only pairs are involved, and the form of simple paths (referred to as \textit{chains}) when a singleton donor starts a sequence of exchanges by donating to a patient in a pair. For instance, consider the cycle 4-3-6 depicted in shaded arcs in Figure \ref{fig:RecourseGraph} and the chain 8-1-5 in the same figure, also in shaded arcs. For logistical reasons, upper bounds $\cycleCap$ and $\chainCap$ are imposed on the number of transplants in cycles and chains, respectively. Then, finding an optimal set of transplants in the compatibility graph is known as the \textit{kidney exchange problem} (KEP). 

%
Confirmation of organ compatibility is a critical aspect to KEP.  A kidney transplant is compatible if a prospective recipient has no presence of \textit{antibodies of importance}, which in addition to ABO blood group antibodies, correspond to those that are directed against a potential donor's human leukocyte antigens (HLAs) \citep{Bhaskaran2022}.  HLAs are the main determinants of an organ rejection \citep{Tait2016}. A \textit{crossmatch test} is used to determine the immunologic risk of a recipient with respect to a potential donor \citep{Bhaskaran2022}. In kidney transplantation, there are two common types of crossmatch tests: physical crossmatch and virtual crossmatch. The former involves mixing a patient's serum with a donor's cells and concluding whether the recipient's cells attack the donor's cells. The latter relies on HLA typing of the donor and anti-HLA assessment of the recipient. Physical crossmatch tests are costly and time-consuming, while virtual crossmatch match tests rely on precise and complete donor HLA typing, which can be difficult to confirm in practice.
%Because a virtual crossmatch relies on precise and complete donor HLA typing, which can be hard to confirm in practice, \KPDPs\ use virtual crossmatch tests in combination with physical crossmatch tests to determine compatibility. A physical crossmatch test is costly, time-consuming  and logistically challenging. 
Thus, \KPDPs\ select a set of transplants based on ``believed'' compatibilities given by the virtual crossmatch results, and confirm (or rule out) viability through a physical crossmatch test only after it is decided that a particular donor will donate to a particular patient. As a result, only a portion of the initially planned transplants may actually take place. Because the transplant operations in a cycle are performed simultaneously in practice, the failure of any of its elements leads to the cancellation of all transplants in that cycle. Chains, on the other hand, are cut short at the pair preceding the first failed transplant. \cite{Dickerson2019} reported that for selected transplants from the UNOS program between 2010--2012, $\approx$93\% did not proceed to transplant. Of those non-successful transplants, 44\% had a failure reason (e.g., failed crossmatch result or patient/donor drop-out) that caused the cancellation of the other 49\% of non-successful transplants. 
%36\% of those 44\%  failed due to a \textit{positive crossmatch result}, i.e., antibodies of importance were detected in the recipient. The other failure reasons were associated to vertices, such as a patient/donor drop-out and sickness \citep{Dickerson2019}.

Some \KPDPs\ decide to relocate pairs belonging to failed exchanges into new cycles and chains to repair the matching. Such re-arrangements depend on specific characteristics of each \KPDP, and follow what is known as a \textit{recourse policy}. Noting that (i) \KPDPs\ that experience high rates of non-successful transplants could benefit from planning for failure before selecting matches, (ii) there is no distributional knowledge that accurately explains how these failures occur, and (iii) previous studies suggest that failure rate between vertices and arcs can be non-homogeneous, we summarize the contributions of this work as follows:

\begin{enumerate}
    \item We study a two-stage robust optimization framework with non-homogeneous failure between vertices and arcs.
    \item We present a general solution framework for any recourse policy whose recourse solution set is finite upon selection of a first-stage set of transplants.
    \item We introduce two feasibility-seeking reformulations of the second stage.
    \item \dma{We compare our framework to state-of-the-art algorithms and find significant computational and solution quality improvements.}
\end{enumerate}

The remainder of this document is organized as follows. Section \ref{LitReview} presents a collection of related works. Section \ref{Preliminaries} establishes the problem we address. Sections \ref{RobustModels} and \ref{SecondStage} present the first and second stage formulations, respectively. Section \ref{SolSecondStage} presents the full algorithmic framework. Section \ref{Experiments} shows computational results. Lastly, Section \ref{sec:Conclusion} draws some conclusions and future work.


